Evaluate On-the-job Learning Dialogue Systems and a Case Study for Natural Language Understanding

On-the-job learning consists in continuously learning while being used in production, in an open environment, meaning that the system has to deal on its own with situations and elements never seen before. The kind of systems that seem to be especially adapted to on-the-job learning are dialogue systems, since they can take advantage of their interactions with users to collect feedback to adapt and improve their components over time. Some dialogue systems performing on-the-job learning have been built and evaluated but no general methodology has yet been defined. Thus in this paper, we propose a first general methodology for evaluating on-the-job learning dialogue systems. We also describe a task-oriented dialogue system which improves on-the-job its natural language component through its user interactions. We finally evaluate our system with the described methodology.

==> algo_NLU_update_strategy_STM.tex <==
\begin{algorithm}
\caption{Natural Language Understanding update strategy through Short Term Memory}\label{alg:nlu_update_stm}
\hspace*{\algorithmicindent} \textbf{Input:} user's utterance u \\
\hspace*{\algorithmicindent} \textbf{Output:} concepts detected in u
\begin{algorithmic}[1]
\Procedure{get\_concepts}{$u$}
\State $concepts_{model} = get\_concepts\_from\_model(u)$
\State $concepts_{stm} = get\_concepts\_from\_stm(u)$
\State initialize $concepts$ as an empty list of concepts
\If{$concept_{stm}$}
    \For{$c_{model}$ in $concepts_{model}$}
        \For{$c_{stm}$ in $concepts_{stm}$}
            \If{$c_{model}.mention == c_{stm}.mention$ and $c_{model}.type == c_{stm}.type$}
                \State add $c_{model}$ to $concepts$
            \ElsIf{$c_{model}.mention == c_{stm}.mention$ and is\_negative($c_{model}.type$)}
                \State add (negative($c_{stm}.type$), $c_{stm}.mention$) to $concepts$
            \ElsIf{$c_{model}.mention$ in $c_{stm}.mention$}
                \State add $c_{stm}$ to $concepts$
            \ElsIf{$c_{stm}.mention$ in $c_{model}.mention$}
                \If{$c_{model}.mention$ in KB}
                    \State add $c_{model}$ to $concepts$
                \Else
                    \State add $c_{stm}$ to $concepts$
                \EndIf
            \EndIf
        \EndFor
        \If{nothing added to concepts}
            \State add $c_{model}$ to $concepts$
        \EndIf
    \EndFor
\Else
    \State $concepts = concepts_{model}$ 
\EndIf
\State \textbf{return} $concepts$
\EndProcedure
\end{algorithmic}
\end{algorithm}

